Exploring Representation of Horn Clauses using GNNs (Extended Technical Report)

Learning program semantics from raw source code is challenging due to the complexity of real-world programming language syntax and due to the difficulty of reconstructing long-distance relational information implicitly represented in programs using identifiers. Addressing the first point, we consider Constrained Horn Clauses (CHCs) as a standard representation of program verification problems, providing a simple and programming language-independent syntax. For the second challenge, we explore graph representations of CHCs, and propose a new Relational Hypergraph Neural Network (R-HyGNN) architecture to learn program features. We introduce two different graph representations of CHCs. One is called constraint graph (CG), and emphasizes syntactic information of CHCs by translating the symbols and their relations in CHCs as typed nodes and binary edges, respectively, and constructing the constraints as abstract syntax trees. The second one is called control- and data-flow hypergraph (CDHG), and emphasizes semantic information of CHCs by representing the control and data flow through ternary hyperedges. We then propose a new GNN architecture, R-HyGNN, extending Relational Graph Convolutional Networks, to handle hypergraphs. To evaluate the ability of R-HyGNN to extract semantic information from programs, we use R-HyGNNs to train models on the two graph representations, and on five proxy tasks with increasing difficulty, using benchmarks from CHC-COMP 2021 as training data. The most difficult proxy task requires the model to predict the occurrence of clauses in counter-examples, which subsumes satisfiability of CHCs. CDHG achieves 90.59% accuracy in this task. Furthermore, R-HyGNN has perfect predictions on one of the graphs consisting of more than 290 clauses. Overall, our experiments indicate that R-HyGNN can capture intricate program features for guiding verification problems.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = pdflatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto


==> sections/7-discussion.tex <==


\section{Discussion}

In many programming language-related fields, such as program verification and synthesis, end-to-end learning frameworks have been applied to learn program features and archive promising results. For instance, LambdaNet~\cite{wei20206lambdanet} represent the program by the \emph{type dependency graph} and learns to infer type annotations, \cite{DBLP:journals/corr/abs-1711-00740} represents program syntactic and semantic structure by graph and learns to reason over program structure. Code2Inv~\cite{CodeToInv} represents the program to a graph consisting of ASTs with terminal and nonterminal nodes and learns to generate loop invariants. They all use message-passing GNNs to learn the program features from the corresponding graph representations.

However, it is unclear which part of the end-to-end frameworks has the most contribution to learning the program features.   
In this work, we did not apply \hyperedgeGNN to generate or select concrete heuristics to solve program verification or synthesis problems. Instead, we systematically explore two critical components for learning program features (i.e., graph representation for CHCs and GNN structure). In particular, the experimental results in Tasks 3, 4, and 5 (the performance of \HyperedgeHornGraphAbbrev is better than that of \layerHornGraph) show that the graph representation should emphasize semantics(e.g., control and data flow) explicitly rather than include the semantics in highly structured syntax, but in Tasks 1 and 2 vice versa. Therefore, we believe the task-tailored graph representation always achieves better performance.
%since the CHC may encode problems from different systems, \layerHornGraphSpace and \HyperedgeHornGraphAbbrevSpace that are designed to describe the program features may not suit all problems.
For example, the two graph representations of CHCs are too redundant to the first three tasks because they do not need the constraint information of CHCs. Therefore, our framework performs better by pruning redundant parts for the graph representation. We supply additional experiments on task 3, in which we define a pruned graph representation\footnote{\url{https://github.com/ChenchengLiang/Horn-graph-dataset/tree/main/example-analysis/task3-pruned}} which only contains the transition information between the relation symbols. i.e., we only draw relation symbols as nodes with label $rs$ and connect them according to the implications in CHCs with a typed edge. With the tailored graph representation, the accuracy of Task 3 further approximates 100\%.

In addition, even though it is hard to know how to customize the two graph representations to a particular task (i.e. we do not know the which program features correspond to which application), we still can use \layerHornGraphSpace and \HyperedgeHornGraphAbbrev as the baseline and try the variations of them to improve the learning results. For instance, We can add reversed edges if we think there is an interaction between these two types of nodes, or we can combine different types of edges to a new typed edge to represent some specific semantics.


%Except for customizing the graph representation and fine-tuning the parameters for different tasks, our framework has more potential. 
Due to the exploding model complexity, the trainable parameters explode for many famous models in different areas. For example, the trainable parameters grow from around 11 million in Resnet18~\cite{DBLP:journals/corr/HeZRS15}  to 175 billion in GTP-3~\cite{DBLP:journals/corr/abs-2005-14165}. However, with the parameters described in section~\ref{trainingModel}, our framework only has around 2 million and 2.2 million trainable parameters for \layerHornGraph and \HyperedgeHornGraphAbbrev, respectively. Moreover, the training dataset only contains a few thousand problems, which suggests we do not need a very big dataset and an extremely large number of parameters to have good results.
%as long as the distribution between the train and test set is similar.
%Both aspects indicate that the combination of graph representation and GNNs has great potential for learning structured information.

One limitation in this framework is that the maximum graph size that the \hyperedgeGNN can handle is limited by the memory size. It is not a trivial implementation problem. One way to handle it is to split the CHCs into multiple subsets. However, this does not affect our conclusion that our framework has good performance for learning program features under challenging tasks.




==> sections/formal-definition-CDHG.tex <==


\section{Formal definition and an algorithm to construct a \HyperedgeHornGraphAbbrev}
\newcommand{\icon}[2][0.5cm]{\begin{minipage}{#1}\includegraphics[width=#1]{#2}\end{minipage}}

\paragraph{Formal definition of \HyperedgeHornGraphAbbrev.}
A \HyperedgeHornGraphAbbrev $HG=(V,\mathit{HE},R^{\HyperedgeHornGraphAbbrev},X^{\HyperedgeHornGraphAbbrev},\ell)$ consists of a set of nodes $v\in V$, a set of typed hyperedge $\mathit{HE} \in V^{*} \times R^{\HyperedgeHornGraphAbbrev}$ where $V^{*}$ is a list of node from $V$, a set of node types $x\in X^{\HyperedgeHornGraphAbbrev}$ (Table~\ref{Hyperedge-Horn-graph-node-definition}),a set of edge types $r\in R^{\HyperedgeHornGraphAbbrev}$ (Table~\ref{Hyperedge-Horn-graph-edge-definition}), and a map $\ell: v\rightarrow x$. %$V$ and $X$ have the same length.
Here, $(v_{1},v_{2},\cdots,v_{n},r) \in HE$ denotes a hyperedge for a list of nodes $(v_{1},\cdots,v_{n})$ with edge type $r$. The node types are used to generate the initial feature $x_{v}$, a real-valued vector, in \hyperedgeGNN.  %$N_{v}^{r}$ represents a set of nodes which contains neighbors of $v$ in edge type $r$.

The guarded $\textit{CFHE}$ is a typed hyperedge $(v_{1},\cdots, v_{n},g,\textit{CFHE}) \in \textit{HE}$, where the type of $v_{1},\cdots,v_{n}$ is $rs$. Since \hyperedgeGNN has more stable performance with fixed number of node in one edge type, we transform the hyperedge $(v_{1},\cdots, v_{n},g,\mathit{CFHE}) \in HE$ with variable number of nodes to a set of ternary hyperedges (i.e., $\{(v_{1},v_{2},g,$ $\mathit{CFHE}),(v_{1},v_{3},g,\mathit{CFHE}),\cdots,(v_{1},v_{n},g,\mathit{CFHE})\}$).

The guarded \textit{DFHE} is a typed ternary hyperedge $(v_{i},v_{j},g, \mathit{DFHE}) \in \mathit{HE}$, where $v_{i}$'s type is $rsa$ and $v_{j}$'s type could be one of $\{op,c,v\}$.





\begin{table*}[tb]
\caption{Node types for the \HyperedgeHornGraphAbbrev. Note that Tables~\ref{layer-Horn-graph-node-definition} and~\ref{Hyperedge-Horn-graph-node-definition} use some same node types because they represent the same elements in the CHC. Some abstract nodes, such as \textit{initial} and \textit{guard}, do not have concrete symbol names since they do not directly associate with any element in the CHCs.} \label{Hyperedge-Horn-graph-node-definition}
\begin{tabular}{lp{5cm}lp{1cm}}
\hline
Node types $X^{CDHG}$ & Explanation & Elements in CHCs & Shape\\
\hline
\textit{relation symbol} ($rs$)  & Relation symbols in head or body  &  $L$ & \icon{graph/process}    \\
\textit{initial}  &  Initial state &   $\emptyset$  & \icon{graph/process}\\
\textit{false}  &   \textit{false} state   &   \textit{false}    & \icon{graph/process}      \\
\textit{relation symbol argument} ($rsa$)  & Arguments of the relation symbols &   $x, y$  & \icon{graph/circle} \\
\textit{variables} ($var$)   & Free variables  &   $n$  & \icon{graph/circle}  \\
\textit{operator} ($op$)    &  Operators over a theory &   =, +     & \icon{graph/square}  \\
\textit{constant} ($c$)    &   Constant over a theory  &  0, 1, $true$  & \icon{graph/round-rectangular}\\
\textit{guard} ($g$) & Guard for \textit{CFHE} and \textit{DFHE}  & $\emptyset$ & \icon{graph/square}\\
%TEMPLATE    &   templates  &  template1,template2   \\
%predicate  & initial predicate (learning target) & predicate\_0 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[tb]
\caption{Edge types for the \HyperedgeHornGraphAbbrev.  $rs, rsa, var, op, c, etc.$ are node types from Table~\ref{Hyperedge-Horn-graph-node-definition}.} \label{Hyperedge-Horn-graph-edge-definition}
\begin{tabular}{p{2.8cm}p{1.5cm}p{3.5cm}p{5cm}}
\hline
Edge type $R^{CDHG}$ & Edge arity & Definition & Explanation\\
\hline
Control Flow Hyperedge (\textit{CFHE})  & Ternary  &  $(rs_{1},rs_{2}~|~\textit{false},g,$ $\textit{CFHE})$ & Connects the $rs$ node in body and head, and abstract \textit{guard} node
%which connects the roots of the control flow sub-formulas. 
\\
\hline
Data Flow Hyperedge (\textit{DFHE}) & Ternary &  $(a,op~|~c~|~var,g, \textit{DFHE})$ & Connects the root node of right-hand and left-hand side of data flow sub-formulas, and a abstract \textit{guard} node
%which connects the root of control flow sub-formulas. 
\\
\hline
Guard (\textit{Guard})  & Binary  &   $(op~|~c,g,\textit{Guard})$ & Connects all roots of ASTs of control flow sub-formulas and the $guard$ node \\
\hline
Relation Symbol Argument (\textit{RSA})  & Binary & $(a,rs,\textit{RSA})$ & Connects $rsa$ nodes and their $rs$ node \\
\hline
AST\_left ($A_{l}$)   & Binary  & $(op,op~|~var~|~c ,A_{l})$ & Connects left-hand side element of a binary operator or an element from a unary operator \\
\hline
AST\_right ($A_{r}$)   & Binary  & $(op,op~|~var~|~c,A_{r})$ & It connects right-hand side element of a binary operator \\
%EqTerm   & binary  &  Connect root of template formula to the corresponding predicate. \\
%InEqTerm  & binary  &  Connect root of template formula to the corresponding predicate. \\
%template   & binary  &  Connect root of template formula to the corresponding predicate. \\
%predicate  & binary  &  Connect PREDICATE node from Horn clauses and predicate nodes from initial predicates. \\
%predicate\_AST (pAST)  & binary  &  Connect AST components in initial predicates. \\
%data   & binary  &   Connect AST components in data flow formulas.  \\
\hline
\end{tabular}
\end{table*}



\paragraph{An abstract example of \HyperedgeHornGraphAbbrev.}
Except for the concrete example, we give a abstract example to describe how to construct the \HyperedgeHornGraphAbbrev.
After the preprocessings (normalization and splitting the constraint to guard and data flow sub-formulas), the CHC $H \leftarrow B_{1}  \wedge \cdots \wedge B_{n} \wedge \varphi$ in Section~\ref{section-banckground} can be re-written to
\begin{equation}\label{horn-clause-definition-2}
 q_{1}(\bar{t_{1}}) \leftarrow q_{2}(\bar{t_{2}}) \wedge \cdots \wedge q_{k}(\bar{t_{k}}) \wedge g_{1}  \wedge \cdots g_{m} \wedge d_{1} \wedge \cdots d_{n}, (m,n,k \in \mathbb{N}).
\end{equation}

We can construct the corresponding \HyperedgeHornGraphAbbrev using Algorithm~\ref{hyperedge-graph-algorithm}, in which the input is a set of CHC and the output is a \HyperedgeHornGraphAbbrev $HG=(V,\mathit{HE},R^{\HyperedgeHornGraphAbbrev},X^{\HyperedgeHornGraphAbbrev},\ell)$.
The step-wise constructing process for the CHC in~(\ref{horn-clause-definition-2}) is visualized in Figure~\ref{abstract-hyperedge-horn-graph}.


\begin{figure*}[tb]
\centering
  \includegraphics[width=\linewidth]{graph/hyperedge-graph-abstract-definition}\\
  \caption{An example to illustrate how to construct the \HyperedgeHornGraphAbbrev from the CHC in (\ref{horn-clause-definition-2}). Here, $g_{i}^{r}$ and $d_{j}^{r}$ are the AST root node of control flow sub-formula $g_{i}$ and the right-hand side of the data flow sub-formula, respectively. The ``$|$" connected edge type $A_{l}~|~A_{r}$ means the edge could be type $A_{l}$ or $A_{r}$. }\label{abstract-hyperedge-horn-graph}
\end{figure*}


\begin{algorithm*}[tb]
\small
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}
\caption{Construct a \HyperedgeHornGraphAbbrev from CHCs}\label{hyperedge-graph-algorithm}
\SetAlgoLined
\KwData{ Normalized CHCs $\Pi$}
\KwResult{A \HyperedgeHornGraphAbbrevSpace $\mathit{HG}=(V,\textit{HE},R^{\HyperedgeHornGraphAbbrev},X^{\HyperedgeHornGraphAbbrev},\ell)$}
Initialise graph: $V,\textit{HE},\ell=\emptyset,\emptyset,\emptyset$\;

\For{ each clause $C$ in $\Pi$}{
    %//draw initial and false node\;
     Add node $v_{initial}$ and $v_{\mathit{false}}$ with type $\textit{initial}$ and $\mathit{false}$ to $V$. Update map $\ell$\;
    //step 1: construct relation symbols and their arguments as typed nodes and add the $RSA$ edge between them\;
    \For{ each relation symbol $q(\bar{t})$ in $C$ }{
        \If{$v_{q} \notin V$}{
            add a node $v_{q}$ with type $rs$ to $V$. Update map $\ell$\;
            \For{ each argument $t$ in $\bar{t}$ }{
                add a node $v_{q}^{t}$ with type $rsa$ to $V$. Update map $\ell$\;
                add a edge from $v_{q}$ to $v_{q}^{t}$ to with type $\textit{RSA}$ to $\textit{HE}$ ;\
            }
        }
    }
    //step 2: construct ASTs for control flow sub-formulas in the constraints and connects the roots of ASTs to an abstract node with type Guard\;
     %//represent constraint of $C$ in the form $\bigwedge \{g_{1},\cdots,g_{i}\} \wedge \bigwedge \{d_{1},\cdots,d_{i}\}$;\
     add a node $v_{g}$ with type $guard$ to $V$. Update map $\ell$;\
    \For{ each $g_{i}$ }{
        %//build AST for $g_{i}$\;
        \For{ each sub-expression $se$ in $g_{i}$ }{
            \If{$v_{se} \notin V$}{
                add a node $v_{se}$ with type $rsa,var,c,$ or $op$ to $V$. Update map $\ell$\;
            }
            add edge from $v_{se}$ to left and right child of $se$ to $\mathit{HE}$ with type $A_{l}$ and $A_{r}$, respectively\;
        }
        add edge from $g_{i}^{r}$ to $v_{g}$ with type Guard to $\mathit{HE}$, where $g_{i}^{r}$ is the root node of $g_{i}$'s AST\;
    }
    //step 3: construct $\textit{CFHEs}$;\\
    \eIf{$C$'s body $\neq \emptyset$}{
        \For{each relation symbol $q(\bar{t})$ in $C$'s body}{
            add a ternary hyperedge $(v_{q(head)},v_{q(body_{i})},v_{g})$ with type $\mathit{CFHE}$, where $v_{q(head)}$ is the node with type $rs$ or $\mathit{false}$ in the head, and $v_{q(body_{i})}$ is the node with type $rs$ in the body;}
    }{
         add a ternary hyperedge $(v_{q(head)},v_{initial},v_{g})$ with type $\textit{CFHE}$ to $\mathit{HE}$;\
    }

    \For{ each $d_{j}$ }{
        //step 4: construct AST for right-hand side of data flow sub-formula $d_{j}$ \;
        \For{ each sub-expression $se$ in right-hand side of $d_{j}$ }{
            \If{$v_{se} \notin V$}{
                add a node $v_{se}$ with type $rsa,var,c,$ or $op$ to $V$. Update map $\ell$\;
            }
            add edge from $v_{se}$ to left and right child of $se$ to $\textit{HE}$ with type $A_{l}$ or $A_{r}$ \;
        }
        //step 5: construct $\textit{DFHEs}$\;
        add a ternary hyperedge $(v_{q}^{t},d_{j}^{r},v_{g})$ with type $\textit{DFHE}$ to $\textit{HE}$, where $v_{q}^{t}$ is the left-hand side element of $d_{j}$ (a node with type $rsa$) and $d_{i}^{r}$ is the root node of $d_{i}$'s AST (a node with type $rsa,var,c$ or $op$ )\;
    }
}
\Return{$V,\textit{HE},\ell$}
\end{algorithm*}




==> sections/formal-definition-constraint-graph.tex <==


\section{Formal definition and an algorithm to construct a \layerHornGraph}
\newcommand{\icon}[2][0.5cm]{\begin{minipage}{#1}\includegraphics[width=#1]{#2}\end{minipage}}

\paragraph{Formal definition of \layerHornGraphSpace.}
A \layerHornGraphSpace $CG=(V,\mathit{BE},R^{CG},X^{CG},\ell)$ consists of a set of nodes $v\in V$, a set of typed binary edges  $\mathit{BE} \in V \times V \times R^{CG}$, a set of edge types $r \in R^{CG}$ (Table~\ref{layer-Horn-graph-edge-definition}), a set of node types $x\in X^{CG}$ (Table~\ref{layer-Horn-graph-node-definition}), and a map $\ell: v \rightarrow x$.
Here, $(v_{1},v_{2},r) \in \mathit{BE}$ denotes a binary edge with edge type $r$. The node types are used to generate the initial feature $x_{v}$, a real-valued vector in \hyperedgeGNN.




\begin{table*}[tb]
\caption{Node types for \layerHornGraph. The shape corresponds to the shape of nodes in Figure~\ref{layer-graph-step-example} and is only used for visualizing the example.} \label{layer-Horn-graph-node-definition}
\begin{tabular}{p{2.5cm}lp{4cm}lp{1cm}}
\hline
Node types $X^{\LayerHornGraphsAbbrev}$ & Layer & Explanation &  Elements in CHCs & Shape \\
\hline
 \textit{relation symbol} ($rs$) & Predicate layer & Relation symbols in head or body  &  $L$   & \icon{graph/process}   \\
 \textit{false}  & Predicate layer &  \textit{false} state  &   \textit{false}       & \icon{graph/process}     \\
 \textit{relation symbol argument} ($rsa$) & Predicate layer  & Arguments of the relation symbols &   x, y   & \icon{graph/circle}  \\
 \textit{clause} ($cla$) & Clause layer &  Represent clause as a abstract node  & $\emptyset$       & \icon{graph/process}     \\
 \textit{clause head} ($ch$) & Clause layer &  Relation symbol in head  &  $L$          & \icon{graph/process}  \\
 \textit{clause body} ($cb$) & Clause layer &  Relation symbol in body  &  $L$         & \icon{graph/process}   \\
 \textit{clause argument} ($ca$)  & Clause layer &  Arguments of relation symbol in head and body  &   $x,y$      & \icon{graph/circle}      \\
 \textit{variable} ($var$) & Constraint layer & Free variables  &  n   & \icon{graph/circle}  \\
 \textit{operator} ($op$) & Constraint layer  &  Operators over a theory &   =, -      & \icon{graph/square}   \\
 \textit{constant} ($c$)  & Constraint layer &   Constants over a theory &  0, 1, $\textit{true}$   & \icon{graph/round-rectangular} \\
%TEMPLATE    &   templates  &  template1,template2   \\
%predicate  & initial predicate (learning target) & predicate\_0 \\
\hline
\end{tabular}
\end{table*}


\begin{table*}[tb]
\caption{Edge types for \layerHornGraph. Here, $rs,rsa,cla$, etc. are node types described in Table~\ref{layer-Horn-graph-node-definition}.Here, ``$|$" means ``or". For example, $c~|~op~|var$ means this node could be node with type $c$, $op$, or $var$.}
\label{layer-Horn-graph-edge-definition}
\begin{tabular}{p{2.8cm}p{2.8cm}p{3.5cm}p{4cm}}
\hline
Edge type $R^{\LayerHornGraphsAbbrev}$ & Layer & Definition & Explanation \\
\hline
Relation Symbol Argument (\textit{RSA})  & Predicate layer & ($rs,rsa, \textit{RSA}$)  &  Connects relation symbols and their arguments \\
\hline
Relation Symbol Instance (\textit{RSI})  & Between predicate and clause layer & $(rs,ch,\textit{RSA})~|~(cb,rs,\textit{RSA})$  & Connects relation symbols with their head and body\\
\hline
Argument~Instance (\textit{AI})  &  Between predicate and clause layer & ($pa,ca,\textit{AI}$)  &  Connects relation symbols and their arguments \\
\hline
Clause~Head (\textit{CH})  &  Clause layer & $(cla,ch,\textit{CH})$  &  Connect $clause$ node to its head  \\
\hline
Clause~Body (\textit{CB})  &  Clause layer & $(cb,cla,\textit{CB})$  &  Connect the $clause$ node to its body  \\
\hline
Clause Argument (\textit{CA})  & Clause layer & $(ca,cb,\textit{CA})~|~(ch,ca,\textit{CA})$ &   Connect $ch$ or $cb$ nodes with corresponding $ca$ nodes \\
\hline
Guard (\textit{GUARD})  &  Between clause and constraint layer & $(c~|~op,cla,\textit{GUARD})$ &  Connect the root node of the AST to corresponding $clause$ node \\
\hline
Data (\textit{DATA})  &  Between clause and constraint layer & $(var,ca,\textit{DATA})$  &  Connect $ca$ nodes to corresponding $var$ nodes AST\\
\hline
AST~sub-term ($A_{st}$) & Constraint layer & $(c~|~var~|~op,op,A_{st})$  & Connect nodes within AST  \\
\hline
\end{tabular}
\end{table*}


\paragraph{An abstract example of \layerHornGraphSpace.}
Except for the concrete example, we give a abstract example to describe how to construct the \layerHornGraph.
First, the CHC $H \leftarrow B_{1}  \wedge \cdots \wedge B_{n} \wedge \varphi$ in Section~\ref{section-banckground} can be re-written to
\begin{equation}\label{horn-clause-definition-3}
 q_{1}(\bar{t_{1}}) \leftarrow q_{2}(\bar{t_{2}}) \wedge \cdots \wedge q_{k}(\bar{t_{k}}) \wedge \varphi_{1}  \wedge \cdots \varphi_{n}, (n,k \in \mathbb{N}),
\end{equation}
where $\varphi_{1} \cdots \varphi_{k}$ are sub-formulas for constraint $\varphi$. Notice that since there is no normalization for the original CHCs, the same relation symbols can appear in both head and body (i.e., $q_{1}, q_{2}, \cdots, q_{k}$ may equal to each other).


Then, we can construct a \layerHornGraph using Algorithm~\ref{layer-graph-algorithm}, in which the input is a set of CHC and the output is a \layerHornGraph $CG=(V,\mathit{BE},R^{CG},X^{CG},\ell)$.
The step-wise constructing process for the CHC in Eq.~(\ref{horn-clause-definition-3}) is visualized in Figure~\ref{abstract-layer-horn-graph}.

\begin{figure*}[tb]
\centering
  \includegraphics[width=\linewidth]{graph/layer-graph-abstract-definition}\\
  \caption{An example to illustrate how to construct the \LayerHornGraph from the CHC in (\ref{horn-clause-definition-2}). Here, $\varphi_{i}^{r}$ is the AST root node $\varphi_{i}$.}\label{abstract-layer-horn-graph}
\end{figure*}


\begin{algorithm*}[tb]
\small
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}
\caption{Construct a \layerHornGraphSpace from CHCs}\label{layer-graph-algorithm}
\SetAlgoLined
\KwData{ Simplified CHCs $\Pi$}
\KwResult{A \layerHornGraph $\textit{CG}=(V,\textit{BE},R^{CG},X^{CG},\ell)$}
Initialise graph: $V,\textit{BE},\ell=\emptyset,\emptyset,\emptyset$\;

\For{ each clause $C$ in $\Pi$}{
    //step 1: construct the predicate layer\;
    \For{ each relation symbol $q(\bar{t})$ in $C$ }{
        \If{$v_{q} \notin V$}{
            //construct a $rs$ node\;
            add a node $v_{q}$ with type $rs$ to $V$. Update map $\ell$; 
            //construct $rsa$ nodes and connect them to the $rs$ node\;
            \For{ each argument $t$ in $\bar{t}$}{
                add a node $v_{q}^{t}$ with type $rsa$ to $V$. Update map $\ell$\;
                add a edge from $v_{q}$ to $v_{q}^{t}$ to with type $\textit{RSA}$ to $\textit{BE}$ ;\
            }
        }
    }
    //step 2: construct the clause layer\;
    %//draw \textit{clause} node\;
    add a node $v_{clause}$ with type $clause$ to $V$. Update map $\ell$;\ 
    %//draw the relation symbol in head and its arguments\;
    add a clause head node $v_{q}^{h}$ with type $ch$ to $V$ for the relation symbol in $C$' head. Update map $\ell$\;
    add a edge from $v_{clause}$ to $v_{q}^{h}$ with type $\textit{CH}$ to $\textit{BE}$ \;
    \For{ each argument $t$ in $\bar{t}$ }{
        add a node $v_{q}^{h,t}$ with type $ca$ to $V$. Update map $\ell$\;
        add a edge from $v_{q}^{h}$ to $v_{q}^{h,t}$ with type $\textit{CA}$ to $\textit{BE}$ \;
    }
    %//draw relation symbols in body and their arguments\;
    \For{ each relation symbol $q(\bar{t})$ in $C$' body }{
        add a clause body node $v_{q}^{b}$ with type $cb$ to $V$. Update map $\ell$ \;
        add a edge from $v_{q}^{b}$ to $v_{clause}$ to with type $\textit{CB}$ to $\textit{BE}$ \;
        \For{ each argument $t$ in $\bar{t}$ }{
            add a node $v_{q}^{b,t}$ with type $ca$ to $V$. Update map $\ell$\;
            add a edge from $v_{q}^{b,t}$ to $v_{q}^{t}$ to with type $\textit{CA}$ to $\textit{BE}$ \;
        }
    }
    //step 3: construct the constraint layer\;
    \For{ each sub-expression $\phi_{i}$ in the constraint}{
        %//build AST for $\phi_{i}$\;
        \For{ each sub-expressions $se$ in $\phi_{i}$ }{
            \If{$v_{se} \notin V$}{
                add a node $v_{se}$ with type $rsa,var,c$ or $op$ to $V$. Update map $\ell$\;
            }
            add edge from $v_{se}$ to the left and right child of $se$ to $\textit{BE}$ with type $A_{st}$\;
        }
    }
    //step 4: add connection between three layers\;
    %// add relation symbol instance ($\mathit{RSI}$) edge between predicate layer and clause layer\;
    \For{ each relation symbol node $v_{q}$ in predicate layer with type $rs$ }{
        add edge $(v_{q},v_{q}^{h})$ or $(v_{q}^{b},v_{q})$ to $\mathit{BE}$ with type $RSI$\;
    }
    %// add argument instance ($\mathit{AI}$) edge from predicate layer to clause layer\;
    \For{ each argument node $v_{q}^{t}$ in predicate layer with type $rsa$ }{
        add edge $(v_{q}^{t},v_{q}^{h,t})$ or $(v_{q}^{b,t},v_{q}^{t})$ to $\textit{BE}$ with type $AI$\;
    }
    %// add Guard edge from constraint layer to clause layer\;
    \For{ each root node of sub-expression $v_{\phi_{i}^{r}}$ }{
        add edge $(v_{\phi_{i}^{r}},v_{clause})$ to $\textit{BE}$ with type Guard\;
    }
    %// add Data edge from constraint layer to clause layer\;
    \For{ each node $v_{se}$ in AST tree with type $v$; \text{if} $v_{se}$ is an argument node }{
        add edge $(v_{se},v_{q}^{h,t})$ or $(v_{q}^{b,t},v_{se})$ to $\textit{BE}$ with type Data\;
    }
}
\Return{$V,\textit{HE},\ell$}
\end{algorithm*}


